Competition Between Regulation-Providing and Fixed-Power Charging Stations for Electric Vehicles

This paper models a non-cooperative game between two EV charging stations. One is a fixed-power charging station purchasing electricity from the grid at wholesale price and reselling the energy to EV owners at a higher retail price; the other is regulation-providing and varies the recharging power level of its clients to provide regulation services to the grid, so its profit comes from both EV owners (who buy energy) and the grid (which pays for regulation services). Users are reluctant to charging power variations and prefer shorter overall charging times, hence regulation-providing charging has to be cheaper than fixed-power charging. We analyze the competition among those charging providers, and examine the performance at the equilibrium in terms of user welfare, station revenue and electricity prices. As expected, competing stations provide users with lower charging prices than when both charging solutions are offered by a monopolistic provider. Moreover, while competition benefits users, it also benefits the grid in that the amount of regulation services increases significantly with respect to the monopolistic case.

==> DataJuly.tex <==
\addplot[only marks, mark=o, blue] coordinates{	
                (1.74069767441860,0)  
                (1.20930232558140,0.335581395348837)  
                (1.20930232558140,0.340930232558140)  
                (1.20930232558140,	0.340930232558140)  
                (0.851627906976744,0.335581395348837)  
                (0.744186046511628,0.696976744186047)  
                (0.744186046511628,0.696976744186047)  
                (0.765116279069767,0.696976744186047)  
                (0.765116279069767,0.696976744186047)  
                (1.71534883720930,0.696976744186047)  
                (1.71534883720930,0.696976744186047)  
                (1.35581395348837,0.0465116279069767)  
                (1.35581395348837,0.441860465116279)  
                (1.51162790697674,0.441860465116279)  
                (1.51162790697674,0.133953488372093)  
                (1.58139534883721,0.133953488372093)  
                (1.58139534883721,0.0116279069767442)  
                (1.71860465116279,0)  
                (1.71860465116279,0)  
                (1.84093023255814,0)  
                (1.84093023255814,0)  
                (1.89534883720930,0)  
                (1.89534883720930,0)  
                (2,0)  
                (2,0)  
                (1.22395348837209,0)  
                (1.22395348837209,0)  
                (2.30232558139535,0)  
                (2.30232558139535,0)  
                (2.24581395348837,0)  
                (2.24581395348837,0)  
                (0,0)  
                (0,0)  
                (1.90697674418605,0)  
                (1.90697674418605,0)   
                (1.83720930232558,0)  
                (1.83720930232558,0)  
                (1.81395348837209,0)  
                (1.81395348837209,0)  
                (0,0)  
                (0,0)  
                (1.83720930232558,0)  
                (1.83720930232558,0)  
                (2.32558139534884,0.133953488372093)  
                (2.32558139534884,0)  
                (2.24581395348837,0.0627906976744187)  
                (2.24581395348837,0.133953488372093)  
		};
%\addlegendentry{\scriptsize Price per half hour on 07/20/2015};	
\addplot[only marks,mark=square,red]
		coordinates {
		(1.6628,0.3759)% the average of Jul. 20 2015
		(1.85406666666667,0.0656463414634150)  
		(1.82484146341464,0.0903937499999996)  
		(1.49025000000000,0.258639534883721)  
		(1.32151041666667,0.117562500000000)  
		(1.213708333333334,0.730402439024390)  
		(1.824835365853659,0.742287500000000)  
		};
%\addlegendentry{\scriptsize Average daily price 07/20 - 07/26/2015}; 
